Logical Satisfiability of Counterfactuals for Faithful Explanations in NLI

Evaluating an explanation's faithfulness is desired for many reasons such as trust, interpretability and diagnosing the sources of model's errors. In this work, which focuses on the NLI task, we introduce the methodology of Faithfulness-through-Counterfactuals, which first generates a counterfactual hypothesis based on the logical predicates expressed in the explanation, and then evaluates if the model's prediction on the counterfactual is consistent with that expressed logic (i.e. if the new formula is \textit{logically satisfiable}). In contrast to existing approaches, this does not require any explanations for training a separate verification model. We first validate the efficacy of automatic counterfactual hypothesis generation, leveraging on the few-shot priming paradigm. Next, we show that our proposed metric distinguishes between human-model agreement and disagreement on new counterfactual input. In addition, we conduct a sensitivity analysis to validate that our metric is sensitive to unfaithful explanations.

==> tables/adversarial_examples.tex <==

\begin{table}[!t]

    \begin{minipage}{\linewidth}
   % \vspace{-\baselineskip}
    \begin{minipage}{.2\linewidth}
    \centering
    \includegraphics[width=0.85\textwidth]{images/adv_ex1.pdf} %
    %\label{fig:hypgraph}

    \end{minipage}%
    \begin{minipage}{.8\linewidth}
    \centering
    \Huge
   %    \caption{}%, we abbreviate the latent belief state of the Opinion Holder, $Z^{OH}$ as $Z$ for brevity.}
    \resizebox{.95\textwidth}{!}{%
       
        \begin{tabular}{l|l}
        Hypothesis & Predicted Class \\ 
        \hline
        The man is holding a person & \texttt{E} (0.88)\\
        
        \hline
        The man is holding a stick. & \texttt{E} (\textcolor{red}{0.63}) \\
        \hline
        \noalign{\vskip 2em}  
        \multicolumn{3}{l}{\textbf{Generated Explanation:}}
        \multicolumn{3}{l}{The man is the same as a man holding a stick.} \\
        %\hline
        \end{tabular}}
    
    \end{minipage} 
    \end{minipage}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
%     \begin{minipage}{\linewidth}
%     \begin{minipage}{.2\linewidth}
%     \centering
%     \includegraphics[width=0.85\textwidth]{images/adv_ex2.pdf} %
%     %\label{fig:hypgraph}

%     \end{minipage}%
%     \begin{minipage}{.8\linewidth}
%     \centering
%   %    \caption{}%, we abbreviate the latent belief state of the Opinion Holder, $Z^{OH}$ as $Z$ for brevity.}
%     \resizebox{.95\textwidth}{!}{%
       
%         \begin{tabular}{l|l|l}
%         & Hypothesis & Predicted Class \\ 
%         \hline
%         Original &  He is outside. & \texttt{E} (0.98)\\
        
%         \hline
%         \hline
%         Revised  & He is on a playground. & \texttt{E} (\textcolor{red}{0.25}) \\
%         \hline
%         \noalign{\vskip 2mm}  
%         \multicolumn{3}{l}{\textbf{Generated Explanation:}}
%         \multicolumn{3}{l}{Outside is the same as at a playground.} \\
%         %\hline
%         \end{tabular}}
}
%    \end{minipage} 
%    \end{minipage}

\caption{Example of an explanation which is plausible but not faithful as it decreases the entailment probability from $0.88$ to $0.63$.}
\label{tab:adversarial}
\end{table}

% \begin{table*}[tbp]

==> tables/entailment_table.tex <==
\begin{table}[!t]
\small
\begin{tabular}{lrll}
\hline
& Model Prediction & Expl(Rel) & Hypothesis  \\
\hline
Original & Contradict & $\neg (A \Leftrightarrow B)$ & $B$  \\
Revised & Entailment & $ A \Leftrightarrow A $ & $A$ \\
\hline
\hline
Original & Entailment & $ A \Leftrightarrow B$ &  $B$ \\
Revised & Entailment & $ A \Leftrightarrow A $ & $A$ \\
\hline
\hline 
Original & Neutral & $A \wedge \neg B$ & $B$ \\
Revised & Entailment & $ A \Leftrightarrow A $ & $A$ \\
Revised & Contradict & $A \wedge \neg B$ & $B$ \\
\hline


\end{tabular}
\caption{\small
[Placeholder entailment table - not everything will be used here, full table will go to appendix]
}
%Entailment table for training with contrastive examples. The tautology examples can be constructed for every training data instance regardless of the label. For each gold label in bold, the additional training instances can be constructed based on the provided relation from the original explanation.}

\label{tab:hyp_results}
\end{table}





==> tables/error_analysis.tex <==
\begin{table}[!t]

\begin{tabular}{l|llll}
modelsize & pipeline & exact & abstract & Overall \\
\hline
GPT-Neo-125M & extraction & ?/60 & ?/40 & \\
GPT-Neo-2.7B & extraction & ?/60 & ?/40 & \\
GPT-Neo-125M & replacement & ?/30 & ?/20 & \\
GPT-Neo-2.7B & replacement & ?/30 & ?/20 & \\
\end{tabular}
\end{table}

==> tables/kappa.tex <==
\begin{table}[!h]
\resizebox{\columnwidth}{!}{
\small
\begin{tabular}{l@{\hskip 0.25in}ccc}
    %$y\mapsto y^{\textrm{cf}}$
    $\texttt{C} \mapsto \texttt{E}$  & $\texttt{E} \mapsto \texttt{E}$ & $\texttt{N}_{[A]} \mapsto \texttt{E}$ & $\texttt{N}_{[B]} \mapsto \texttt{N}$ \\
     \toprule
    0.462 & 0.353 & 0.368 & 0.279 
\end{tabular}
}
\caption{Fleiss' kappa for agreement between three human annotators on the counterfactual label grouped by the original label (LHS of $\mapsto$ in header row).}
\label{tab:kohen}
\end{table}

\begin{table}[!h]
\resizebox{\columnwidth}{!}{
 \small
\begin{tabular}{l@{\hskip 0.25in}cccc}
%$y\mapsto y^{\textrm{cf}}$ 
$\texttt{C} \mapsto \texttt{E}$ & $\texttt{E} \mapsto \texttt{E}$ & $\texttt{N}_{[A]} \mapsto \texttt{E}$ & $\texttt{N}_{[B]} \mapsto \texttt{N}$ \\
    %& \texttt{C} & \texttt{E} & \texttt{N}_{[A\backslash B]} & \texttt{N}_{[B\backslash A]}  \\
    \toprule
      0.534 & 0.867 & 0.756 & 0.714 
\end{tabular}
}
\caption{Accuracy of aggregated human label in predicting derived NLI label (RHS of $\mapsto$; \autoref{sec:problem_formulation}).}
\label{tab:agreement}
\end{table}


==> tables/transform_success.tex <==
\begin{table*}[!t]
\small
\begin{tabular}{lllllll}
class label & explanation type & prompt sample type & pipeline & unconverted & context & conversion \\
\hline
entailment & gold & GPT & kmeans & & 960/5254 & \\
entailment & gold & GPT & random & & 1146/5254 & \\
entailment & gold & Regex+GPT & kmeans &  & 880/5254 & \\
entailment & gold & Regex+GPT & random & & 1148/5254 & \\
\hline
entailment & gen & GPT & kmeans & & 1262/4988 & \\
entailment & gen & GPT & random & & 1324/4988 &  \\
entailment & gen & Regex+GPT & kmeans & & 1132/4988 &\\
entailment & gen & Regex+GPT & random & & 1190/4988 & \\
\hline
contradiction & gold & GPT & kmeans & & 587/5643 & \\
contradiction & gold & GPT & random & & 827/5643  & \\
contradiction & gold & Regex+GPT & kmeans & & 593/5643 & \\
contradiction & gold & Regex+GPT & random & & 825/5643  & \\
\hline
contradiction & gen & GPT & kmeans & & 312/4779 & \\
contradiction & gen & GPT & random & & 505/4779 & \\
contradiction & gen & Regex+GPT & kmeans & & 288/4779 & \\
contradiction & gen & Regex+GPT & random & & 444/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H1-I1-L1 & 288/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H1-I1-L0 & 1147/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H1-I0-L1 & 472/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H0-I1-L1 & 1396/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H1-I0-L0 & x/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H0-I1-L0 & x/4779 & \\
contradiction & gen & Regex+GPT & kmeans & H0-I0-L1 & 1900/4779 & \\

\end{tabular}
\end{table*}
